Adversarial Regression. Generative Adversarial Networks for Non-Linear Regression: Theory and Assessment

Adversarial Regression is a proposition to perform high dimensional non-linear regression with uncertainty estimation. We used Conditional Generative Adversarial Network to obtain an estimate of the full predictive distribution for a new observation. Generative Adversarial Networks (GAN) are implicit generative models which produce samples from a distribution approximating the distribution of the data. The conditional version of it (CGAN) takes the following expression: $\min\limits_G \max\limits_D V(D, G) = \mathbb{E}_{x\sim p_{r}(x)} [log(D(x, y))] + \mathbb{E}_{z\sim p_{z}(z)} [log (1-D(G(z, y)))]$. An approximate solution can be found by training simultaneously two neural networks to model D and G and feeding G with a random noise vector $z$. After training, we have that $G(z, y)\mathrel{\dot\sim} p_{data}(x, y)$. By fixing $y$, we have $G(z|y) \mathrel{\dot\sim} p{data}(x|y)$. By sampling $z$, we can therefore obtain samples following approximately $p(x|y)$, which is the predictive distribution of $x$ for a new $y$. We ran experiments to test various loss functions, data distributions, sample size, size of the noise vector, etc. Even if we observed differences, no experiment outperformed consistently the others. The quality of CGAN for regression relies on fine-tuning a range of hyperparameters. In a broader view, the results show that CGANs are very promising methods to perform uncertainty estimation for high dimensional non-linear regression.

==> Theory.tex <==
# Generative Adversarial Networks (GANs)

GANs are a way to approximate any kind of distributions from . They are said to be "adversarial" because they can be presented as two neural networks playing against each others. The Generator generates fake data. The Discriminator learn to distinguish between real data and fake data. It is a simple classifyer trying to be right. The Generator try to produce data that foul the Discriminator. By iteration, the Generator eventually produce fake data undistinguable from the real data.
Actually, Goodfellow himself propose to see it as a cooperarive game.

$G:R^D -> X$
$D:X -> [0, 1]$




# GAN's

We have an unknown density function $p_{r}(x)$ and a dataset containing realizations of this model. We want to use this sample to estimate  $p_{r}(x)$.
The idea is as follow:
 1) We generate some data $z$ from a simple known distribution, typically the standard normal.
 2) We train a function $G(z)$ to simulate as good as possible realizations of x, so that we have $G(z)=x \sim p_g(x)$.
 3) We train a discriminator $D$ to distinguish between $x$ coming from $p_r(x)$ and the one coming from $p_g(x)$

Actually $G$ and $D$ are trained simultaneously through optimization algorithm each of them making one step of optimization after the other. The process is as a game between two players [Note: In fact, it is related to the game theory and Nash equilibrium]. The first player the Generator try to foul the Discriminator by generating sample as close as possible of the real distribution. The discriminator try not to be foul. The better one player becomes, the better the other one has to be in order to succeed in its task.

Let start with the discriminative part. It is a classification task. As shown previously, the loss function for such a case is given by the cross entropy loss function. Pluging in the GAN's notation, the loss function can be written: 
$$ \max\limits_D V(D, G) = \mathbb{E}_{x\sim p_{r}(x)} [ln(D(x))] + \mathbb{E}_{z\sim p_{z}(z)} [ln (1-D(G(z)))] $$

Here, we can apply a change of variable that is not obvious if we do not want to assume that G is invertible (which is not the case with neural networks). Thanks to the Radon–Nikodym theorem, it is possible to write: 
$$ \max\limits_D V(D, G) = \mathbb{E}_{x\sim p_{r}(x)} [ln(D(x))] + \mathbb{E}_{x\sim p_{G}(x)} [ln (1-D(x))] $$
For a fix G(z), we can then find the $D^{\star}_G$ that maximize the loss function: 

$$ D_G^{\star}= \text{arg}\max\limits_D \int p_{r}(x) [ln(D(x))] + p_{g}(x) [ln (1-D(x))] dx$$

Since it is the same as maximizing the integrand, the maximum is obtained where the first derivative is null if the second derivative is negative for all x's. 
$$
\begin{split}
D_G' & = \frac{p_{r}(x)}{D(x)} + \frac{p_{g}(x)}{(1-D(x))}  \\
D_G^{\star} & = \frac{p_{r}(x)}{p_{r}(x)+p_{g}(x)}
\end{split}
$$

By pluging the result into the objective function we have: 
$$
V(D^{\star}, G)= \int p_{r}(x) ln(\frac{p_{r}(x)}{p_{r}(x)+p_{g}(x)}) + p_{g}(x) ln(\frac{p_{g}(x)}{p_{r}(x)+p_{g}(x)}) dx
$$

The general aim of the process is to have a generator mimicking perfectly the true distribution $p_{r}(x)$. Let set then ${p_{r}(x)=p_{g}(x)}$. It implies that that $D_G^{\star}=\frac{1}{2}$. The objective function becomes: 

$$V(D^{\star}, G)= \int p_{r}(x) ln(\frac{1}{2}) + p_{g}(x) ln(\frac{1}{2})dx$$

It is easy to see that $V(D^{\star}, G)= -2ln(2)$ but we would like to do more. The aim is to prove that this minimum can be reached for only one G. 

$$
V(D^{\star}, G) = \int p_{r}(x) ln(\frac{p_{r}(x)}{p_{r}(x)+p_{g}(x)}) + p_{g}(x) ln(\frac{p_{g}(x)}{p_{r}(x)+p_{g}(x)}) dx $$
$$
= \int (ln(2)-ln(2))p_{r}(x) + p_{r}(x) ln(\frac{p_{r}(x)}{p_{r}(x)+p_{g}(x)}) + (ln(2)-ln(2))p_{g}(x) + p_{g}(x) ln(\frac{p_{g}(x)}{p_{r}(x)+p_{g}(x)})dx $$
$$
= -ln(2 \int {p_{r}(x)+p_{g}(x)} dx) + \int p_{r}(x)(ln(2) + ln(\frac{p_{r}(x)}{p_{r}(x)+p_{g}(x)}) + p_{g}(x)(ln(2) + ln(\frac{p_{g}(x)}{p_{r}(x)+p_{g}(x)})dx $$
$$
= -2ln(2) + \int p_{r}(x)(\frac{p_{r}(x)}{(p_{r}(x)+p_{g}(x))/2})dx + \int p_{g}(x)\frac{p_{g}(x)}{(p_{r}(x)+p_{g}(x))/2}dx
$$

By definition of the Kullback-Leibler divergence, we have: 
$$
V(D^{\star}, G) = -2ln(2) + D_{KL}(p_{r}(x)\vert \frac{(p_{r}(x)+p_{g}(x))}{2}) + D_{KL}(p_{g}(x)\vert \frac{(p_{r}(x)+p_{g}(x))}{2})
$$
The Kullback-Leibler divergence is non-negative so we confirm that $-2ln(2)$ is a global minimum. 

And by definition of the the Jenson-Shannon divergence, we obtain: 

$$
V(D^{\star}, G) = -2ln(2) + D_{JS}(p_{r}(x)\vert p_{g}(x)
$$

The Jenson-Shannon divergence is $0$ only when $p_{r}(x)= p_{g}(x)$). 


The main problem with GANs is that they are known to be hard to train. The problems appears when one of the network is too strong for the other. 
If the discriminator becomes too strong, meaning its classifing correctly with high confidence all the observations, the generator would not be able to learn anything. Indeed, if D(G(z)) is close to one, log(1-D(G(z) saturates and its gradient vanish. The author of the original paper propose to avoid it by maximizing log(D(G(z))) instead of minimizing log(1-D(G(z))). By changing the sigh of the new expression the objetive becomes again a minimization problem. The new loss function is then: 
<[\max\limits G \max\limits_D V(D, G) = \mathbb{E}_{x\sim p_{r}(x)} [ln(D(x))] - \mathbb{E}_{z\sim p_{z}(z)} [ln (D(G(z)))]

the gradient of the Generator is van
The most famous reason is the so-called mode collapse. The issue apprears if the 



# Wasserstein GAN (WGAN)

One solution to the mode collapse have been presented by lalalalilala. They propose to change the loss function. The problem with the classic GANs' loss function is that the gradient of $log(D(p_g(x)))$ has a high variance when $p_g(x)$ is close to 1. 
The new cost function lay on the Wasserstein distance also called Earth-Mover distance. The idea is that the distance between two distributions is the minimum distance of density (thought as earth) to move in order that the two distribution matches. Formally the Wasserstein distance is written: 
$$ W(p, q) = \inf_{\gamma \in \Pi(p, q)} \iint\limits_{x,y} \lVert x - y \lVert \gamma (x,y) \, \mathrm{d} x \, \mathrm{d} y  = \inf_{\gamma \in \Pi(p, q)} \mathbb{E}_{(x, y)\sim\gamma}(\left\lVert x-y \right\rVert)  $$


where $\Pi(p, q)$ denotes the set of all joint distribution $\gamma(x, y)$ whose marginals are respectively $p$ and $q$. The above formulation is intractable. 
The authors of the original paper propose then a transformation requiring quite complicated mathematics. For details about it Vincent Herrman wrote a convincing explanation: (https://vincentherrmann.github.io/blog/wasserstein/). The result is that we can also express the former formulation as follow: 

$$W(p_r, p_g) = \frac{1}{K} \sup_{\| f \|_L \leq K} \mathbb{E}_{x \sim p}(f(x)) - \mathbb{E}_{x \sim q}(f(x))$$

The new formulation makes appear the condition $\| f \|_L \leq K$, meaning that $f$ should to be K-Liptschitz continuous. A real function $f: \mathbb{R} \rightarrow \mathbb{R}$ is said K-Liptschitz if there is a real constant $K$ such that 

$$\lvert f(x_1) - f(x_2) \rvert \leq K \lvert x_1 - x_2 \rvert$$ $\forall x_1, x_2 \in \mathbb{R}$$

The idea is to make of the discriminator a family of K-Lipschitz continuous function $f_\theta$. 
It would be then possible to rewrite the loss function of the discriminator as a Wasserstein distance. Assuming that $f_\theta$ is K_Lipschitz, the loss function becomes: 
$$L(p_r, p_g) = W(p_r, p_g) = \max_{\theta} \mathbb{E}_{x \sim p_r}(f_\theta(x)) - \mathbb{E}_{z \sim p_r(z)}(f_\theta(G(z)))$$
So, the discriminator is not a classifier anymore. It is rather a function required to compute Wassstein distance.
The issue is now to keep $f\theta$ being a K-Lipschitz coninuous function so that the above devlopments hold. The trick used is quite simple. It consists in clamping the weight after each update in order that the parameter space keep very compact. Thus, $f_\theta$ is bounded such that the K-Lipschitz continuity is preserved. The weight are clamp in an interval $[-c,c]$, where $c$ is a small value. The autors recommand $c$ being of the order of $10^{-2}$. 

WGANs solve the problem of vanishing or high variance gradients. They offer also a more convincing way of computing distance between distributions for the kind of issue they deal with. The theory is convincing. The problem is that it is not clear that they perform better than classic GAN.

The interest of it... 
